Ground-aware Monocular 3D Object Detection for Autonomous Driving

Estimating the 3D position and orientation of objects in the environment with a single RGB camera is a critical and challenging task for low-cost urban autonomous driving and mobile robots. Most of the existing algorithms are based on the geometric constraints in 2D-3D correspondence, which stems from generic 6D object pose estimation. We first identify how the ground plane provides additional clues in depth reasoning in 3D detection in driving scenes. Based on this observation, we then improve the processing of 3D anchors and introduce a novel neural network module to fully utilize such application-specific priors in the framework of deep learning. Finally, we introduce an efficient neural network embedded with the proposed module for 3D object detection. We further verify the power of the proposed module with a neural network designed for monocular depth prediction. The two proposed networks achieve state-of-the-art performances on the KITTI 3D object detection and depth prediction benchmarks, respectively. The code will be published in https://www.github.com/Owen-Liuyuxuan/visualDet3D

==> secs/pics/arch.tex <==
\begin{figure*}
    \begin{subfigure}[b]{1.0\textwidth}
        \includegraphics[{width=1.0\textwidth}]{secs/pics/Arch.png}
        
    \end{subfigure}
    \caption{\textbf{Network inference structure of YOLOMono3D.}
    The classification branch takes the feature map from ResNet, and it outputs dense prediction on objectness scores for each category and multi-class classification scores for each 3D dimension.
    The regression branch produces dense estimation of the normalized 2D/3D bounding box parameters $[x, y, w, h, cx, cy, z, sin(\alpha), cos(\alpha)]$.
    During inference, we further perform non-max suppression, followed by hill-climbing post optimization to produce final 3D detection results.
   }
    \label{fig:architecture}
\end{figure*}
